Are GRBs the same at high and low redshift?

Due to their highly luminous nature, gamma-ray bursts (GRBs) are useful tools in studying the early Universe (up to z = 10). We consider whether the available subset of Swift high redshift GRBs are unusual when compared to analogous simulations of a bright low redshift sample. By simulating data from the Burst Alert Telescope (BAT; Barthelmy et al. 2005) the light curves of these bright bursts are obtained over an extensive range of redshifts, revealing complicated evolution in properties of the prompt emission such as T90.

==> aas_abbrev.tex <==
\newcommand\aj{AJ}%
          % Astronomical Journal
\newcommand\actaa{Acta Astron.}%
 	  % Acta Astronomica
\newcommand\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{ApJ}%
          % Astrophysical Journal
\newcommand\apjl{ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{BAAS}%
          % Bulletin of the AAS
\newcommand\caa{Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{Icarus}%
  % Icarus
\newcommand\jcap{J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{New A}%
  % New Astronomy
\newcommand\nar{New A Rev.}%
  % New Astronomy Review
\newcommand\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{PASP}%
          % Publications of the ASP
\newcommand\pasj{PASJ}%
          % Publications of the ASJ
\newcommand\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%
          % Sky and Telescope
\newcommand\solphys{Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{Nature}%
          % Nature
\newcommand\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

